Enhancing the Transferability of Adversarial Attacks through Variance Tuning

Deep neural networks are vulnerable to adversarial examples that mislead the models with imperceptible perturbations. Though adversarial attacks have achieved incredible success rates in the white-box setting, most existing adversaries often exhibit weak transferability in the black-box setting, especially under the scenario of attacking models with defense mechanisms. In this work, we propose a new method called variance tuning to enhance the class of iterative gradient based attack methods and improve their attack transferability. Specifically, at each iteration for the gradient calculation, instead of directly using the current gradient for the momentum accumulation, we further consider the gradient variance of the previous iteration to tune the current gradient so as to stabilize the update direction and escape from poor local optima. Empirical results on the standard ImageNet dataset demonstrate that our method could significantly improve the transferability of gradient-based adversarial attacks. Besides, our method could be used to attack ensemble models or be integrated with various input transformations. Incorporating variance tuning with input transformations on iterative gradient-based attacks in the multi-model setting, the integrated method could achieve an average success rate of 90.1% against nine advanced defense methods, improving the current best attack performance significantly by 85.1% . Code is available at https://github.com/JHL-HUST/VT.

==> tables/diversity_gradient_attack_transferability.tex <==
\begin{table*}[tb]
\small
\begin{center}
\begin{tabular}{|l|c|ccccccc|}
\hline
Model & Attack & Inc-v3 & Inc-v4 & IncRes-v2 & Res-101 & Inc-v3$_{ens3}$ & Inc-v3$_{ens4}$ & IncRes-v2$_{ens}$\\
\hline\hline
\multirow{4}{*}{Inc-v3} & MI-DI-FGSM & ~~99.0* & 64.3 & 60.9 & 53.2 & 19.9 & 18.3 &  9.3\\
 & VMI-DI-FGSM & \textbf{~~99.2*} & \textbf{75.2} & \textbf{73.8} & \textbf{67.4} & \textbf{38.9} & \textbf{38.3} & \textbf{22.6}\\
\cline{2-9}
 & NI-DI-FGSM & ~~99.1* & 62.1 & 58.1 & 48.5 & 14.4 & 15.0 &  7.3\\
 & VNI-DI-FGSM & \textbf{~~99.4*} & \textbf{79.0} & \textbf{77.1} & \textbf{69.2} & \textbf{39.7} & \textbf{38.0} & \textbf{22.7}\\
\hline
\multirow{4}{*}{Inc-v4} & MI-DI-FGSM & 72.9 & ~~97.4* & 65.1 & 56.5 & 20.2 & 21.1 & 11.6\\
 & VMI-DI-FGSM & \textbf{82.3} & \textbf{~~98.4*} & \textbf{75.0} & \textbf{68.7} & \textbf{43.8} & \textbf{41.1} & \textbf{30.5}\\
\cline{2-9}
 & NI-DI-FGSM & 70.9 & \textbf{~~99.1*} & 59.1 & 50.5 & 16.8 & 17.2 &  8.4\\
 & VNI-DI-FGSM & \textbf{83.9} & \textbf{~~99.1*} & \textbf{78.0} & \textbf{71.1} & \textbf{44.2} & \textbf{42.2} & \textbf{29.0}\\
\hline
\multirow{4}{*}{IncRes-v2} & MI-DI-FGSM & 70.1 & 63.4 & ~~93.5* & 58.7 & 30.9 & 23.9 & 17.7\\
 & VMI-DI-FGSM & \textbf{76.3} & \textbf{74.8} & \textbf{~~94.8*} & \textbf{69.9} & \textbf{52.7} & \textbf{45.8} & \textbf{41.0}\\
 \cline{2-9}
 & NI-DI-FGSM & 69.2 & 62.0 & ~~96.0* & 54.0 & 21.7 & 18.8 & 12.3\\
 & VNI-DI-FGSM & \textbf{81.4} & \textbf{77.9} & \textbf{~~96.8*} & \textbf{72.9} & \textbf{52.9} & \textbf{45.8} & \textbf{40.9}\\
\hline
\multirow{4}{*}{Res-101} & MI-DI-FGSM & 75.8 & 69.5 & 70.0 & ~~98.0* & 35.7 & 31.6 & 19.9\\
 & VMI-DI-FGSM & \textbf{80.4} & \textbf{76.1} & \textbf{78.0} & \textbf{~~98.5*} & \textbf{54.4} & \textbf{51.1} & \textbf{40.5}\\
 \cline{2-9}
 & NI-DI-FGSM & 74.7 & 69.1 & 68.3 & \textbf{~~98.9*} & 26.9 & 24.9 & 15.1\\
 & VNI-DI-FGSM & \textbf{84.4} & \textbf{79.3} & \textbf{79.8} & ~~98.8* & \textbf{54.6} & \textbf{51.0} & \textbf{39.1}\\
\hline
\end{tabular}
\end{center}
\vspace{-0.3em}
\caption{The success rates (\%) on seven models in the single model setting by various gradient-based iterative attacks enhanced by DIM.}
\label{tab:DIM}
\end{table*}

==> tables/scale_gradient_attack_transferability.tex <==
\begin{table*}[tb]
\begin{center}
\begin{tabular}{|l|c|ccccccc|}
\hline
Model & Attack & Inc-v3 & Inc-v4 & IncRes-v2 & Res-101 & Inc-v3$_{ens3}$ & Inc-v3$_{ens4}$ & IncRes-v2$_{ens}$\\
\hline\hline
\multirow{4}{*}{Inc-v3} & MI-SI-FGSM & \textbf{100.0*} & 69.2 & 66.6 & 62.9 & 30.7 & 31.6 & 17.1\\
 & VMI-SI-FGSM & \textbf{100.0*} & \textbf{86.8} & \textbf{83.8} & \textbf{77.5} & \textbf{55.7} & \textbf{52.3} & \textbf{35.7}\\
\cline{2-9}
 & NI-SI-FGSM & \textbf{100.0*} & 76.3 & 75.7 & 66.9 & 32.5 & 30.8 & 17.0\\
 & VNI-SI-FGSM & \textbf{100.0*} & \textbf{89.7} & \textbf{88.3} & \textbf{82.2} & \textbf{57.9} & \textbf{55.5} & \textbf{37.6}\\
\hline
\multirow{4}{*}{Inc-v4} & MI-SI-FGSM & 80.6 & \textbf{~~99.6*} & 74.2 & 68.8 & 47.8 & 44.8 & 29.1\\
 & VMI-SI-FGSM & \textbf{88.7} & ~~99.5* & \textbf{85.2} & \textbf{78.7} & \textbf{65.2} & \textbf{61.2} & \textbf{47.2}\\
\cline{2-9}
 & NI-SI-FGSM & 86.7 & \textbf{100.0*} & 78.5 & 72.5 & 44.6 & 41.0 & 26.3\\
 & VNI-SI-FGSM & \textbf{91.6} & ~~99.9* & \textbf{88.8} & \textbf{83.9} & \textbf{66.4} & \textbf{64.3} & \textbf{49.0}\\
\hline
\multirow{4}{*}{IncRes-v2} & MI-SI-FGSM & 84.7 & 81.1 & \textbf{~~99.0*} & 76.4 & 56.3 & 48.3 & 42.8\\
 & VMI-SI-FGSM & \textbf{90.2} & \textbf{88.1} & ~~98.7* & \textbf{84.0} & \textbf{73.9} & \textbf{67.0} & \textbf{63.9}\\
 \cline{2-9}
 & NI-SI-FGSM & 87.2 & 80.3 & \textbf{~~99.6*} & 77.2 & 50.0 & 42.9 & 36.1\\
 & VNI-SI-FGSM & \textbf{93.4} & \textbf{90.9} & ~~99.3* & \textbf{87.6} & \textbf{75.0} & \textbf{69.4} & \textbf{65.4}\\
\hline
\multirow{4}{*}{Res-101} & MI-SI-FGSM & 75.2 & 68.9 & 69.0 & \textbf{~~99.7*} & 43.7 & 38.5 & 26.3\\
 & VMI-SI-FGSM & \textbf{84.3} & \textbf{79.6} & \textbf{81.4} & \textbf{~~99.7*} & \textbf{64.2} & \textbf{57.8} & \textbf{44.8}\\
 \cline{2-9}
 & NI-SI-FGSM & 78.2 & 74.7 & 74.0 & \textbf{~~99.8*} & 41.7 & 38.1 & 25.0\\
 & VNI-SI-FGSM & \textbf{87.6} & \textbf{85.8} & \textbf{84.9} & \textbf{~~99.8*} & \textbf{66.3} & \textbf{60.7} & \textbf{47.4} \\
\hline
\end{tabular}
\end{center}
\vspace{-0.5em}
\caption{The success rates (\%) on seven models in the single model setting by various gradient-based iterative attacks enhanced by Scale-Invariant  Method.}
\label{tab:SIM}
\end{table*}

% \begin{table*}
% \begin{center}
% \begin{tabular}{|l|c|ccccccc|}
% \hline
% Model & Attack & Inc-v3 & Inc-v4 & IncRes-v2 & Res-101 & Inc-v3$_{ens3}$ & Inc-v3$_{ens4}$ & IncRes-v2$_{ens}$\\
% \hline\hline
% \multirow{4}{*}{Inc-v3} & MI-SI-FGSM & \textbf{100.0*} & 69.2 & 66.6 & 62.9 & 30.7 & 31.6 & 17.1\\
%  & VMI-SI-FGSM & ~~99.7* & \textbf{87.7} & \textbf{86.4} & \textbf{82.8} & \textbf{67.0} & \textbf{64.2} & \textbf{47.5}\\
% \cline{2-9}
%  & NI-SI-FGSM & \textbf{100.0*} & 76.3 & 75.7 & 66.9 & 32.5 & 30.8 & 17.0\\
%  & VNI-SI-FGSM & \textbf{100.0*} & \textbf{89.6} & \textbf{89.6} & \textbf{85.0} & \textbf{68.9} & \textbf{65.4} & \textbf{48.3}\\
% \hline
% \multirow{4}{*}{Inc-v4} & MI-SI-FGSM & 80.6 & \textbf{~~99.6*} & 74.2 & 68.8 & 47.8 & 44.8 & 29.1\\
%  & VMI-SI-FGSM & \textbf{89.0} & ~~99.4* & \textbf{86.4} & \textbf{81.9} & \textbf{72.8} & \textbf{72.9} & \textbf{58.9}\\
% \cline{2-9}
%  & NI-SI-FGSM & 86.7 & \textbf{100.0*} & 78.5 & 72.5 & 44.6 & 41.0 & 26.3\\
%  & VNI-SI-FGSM & \textbf{92.3} & ~~99.9* & \textbf{89.0} & \textbf{86.2} & \textbf{74.9} & \textbf{74.0} & \textbf{59.8}\\
% \hline
% \multirow{4}{*}{IncRes-v2} & MI-SI-FGSM & 84.7 & 81.1 & \textbf{~~99.0*} & 76.4 & 56.3 & 48.3 & 42.8\\
%  & VMI-SI-FGSM & \textbf{89.0} & \textbf{85.5} & ~~97.5* & \textbf{84.0} & \textbf{76.3} & \textbf{73.9} & \textbf{70.3}\\
%  \cline{2-9}
%  & NI-SI-FGSM & 87.2 & 80.3 & \textbf{~~99.6*} & 77.2 & 50.0 & 42.9 & 36.1\\
%  & VNI-SI-FGSM & \textbf{91.2} & \textbf{88.5} & ~~99.3* & \textbf{87.1} & \textbf{78.4} & \textbf{75.5} & \textbf{71.7} \\
% \hline
% \multirow{4}{*}{Res-101} & MI-SI-FGSM & 75.2 & 68.9 & 69.0 & \textbf{~~99.7*} & 43.7 & 38.5 & 26.3\\
%  & VMI-SI-FGSM & \textbf{83.6} & \textbf{79.3} & \textbf{81.8} & ~~99.5* & \textbf{70.3} & \textbf{67.7} & \textbf{57.8}\\
%  \cline{2-9}
%  & NI-SI-FGSM & 78.2 & 74.7 & 74.0 & ~~99.8* & 41.7 & 38.1 & 25.0\\
%  & VNI-SI-FGSM & \textbf{87.5} & \textbf{83.0} & \textbf{84.1} & \textbf{~~99.9*} & \textbf{73.7} & \textbf{68.4} & \textbf{57.7}\\
% \hline
% \end{tabular}
% \end{center}
% \caption{Attack success rates (\%) on seven models under single model setting by I-FGSM with variations of gradient calculation enhanced by Scale-Invariant  Method.}
% \end{table*}

==> tables/transformation_gradient_attack_transferability.tex <==
\begin{table*}[tb]
\begin{center}
\begin{tabular}{|l|c|ccccccc|}
\hline
Model & Attack & Inc-v3 & Inc-v4 & IncRes-v2 & Res-101 & Inc-v3$_{ens3}$ & Inc-v3$_{ens4}$ & IncRes-v2$_{ens}$\\
\hline\hline
\multirow{4}{*}{Inc-v3} & MI-TI-FGSM & \textbf{100.0*} & 48.8 & 43.6 & 39.5 & 24.8 & 21.3 & 13.2\\
 & VMI-TI-FGSM & \textbf{100.0*} & \textbf{72.1} & \textbf{69.3} & \textbf{58.8} & \textbf{48.1} & \textbf{48.1} & \textbf{36.3}\\
\cline{2-9}
 & NI-TI-FGSM & \textbf{100.0*} & 55.5 & 51.1 & 45.3 & 24.0 & 23.4 & 14.7\\
 & VNI-TI-FGSM & \textbf{100.0*} & \textbf{76.4} & \textbf{73.4} & \textbf{64.6} & \textbf{53.0} & \textbf{50.3} & \textbf{38.1}\\
\hline
\multirow{4}{*}{Inc-v4} & MI-TI-FGSM & 58.6 & \textbf{~~99.6*} & 46.5 & 42.3 & 26.2 & 23.4 & 17.2\\
 & VMI-TI-FGSM & \textbf{76.3} & \textbf{~~99.6*} & \textbf{69.1} & \textbf{59.1} & \textbf{52.1} & \textbf{47.1} & \textbf{42.1}\\
\cline{2-9}
 & NI-TI-FGSM & 66.0 & \textbf{100.0*} & 54.3 & 47.2 & 27.8 & 24.8 & 16.1\\
 & VNI-TI-FGSM & \textbf{80.8} & ~~99.9* & \textbf{72.5} & \textbf{65.3} & \textbf{55.5} & \textbf{50.9} & \textbf{43.3}\\
\hline
\multirow{4}{*}{IncRes-v2} & MI-TI-FGSM & 62.2 & 55.4 & ~~97.4* & 50.5 & 32.8 & 27.6 & 23.3\\
 & VMI-TI-FGSM & \textbf{78.0} & \textbf{73.3} & \textbf{~~97.5*} & \textbf{67.5} & \textbf{59.0} & \textbf{52.8} & \textbf{52.4}\\
 \cline{2-9}
 & NI-TI-FGSM & 68.0 & 60.7 & \textbf{~~98.3*} & 51.8 & 31.9 & 26.1 & 21.2\\
 & VNI-TI-FGSM & \textbf{81.3} & \textbf{77.0} & ~~98.1* & \textbf{70.6} & \textbf{62.2} & \textbf{55.3} & \textbf{53.4}\\
\hline
\multirow{4}{*}{Res-101} & MI-TI-FGSM & 59.3 & 52.1 & 51.8 & \textbf{~~99.3*} & 35.4 & 31.3 & 23.1\\
 & VMI-TI-FGSM & \textbf{73.1} & \textbf{67.9} & \textbf{69.4} & \textbf{~~99.3*} & \textbf{56.7} & \textbf{52.7} & \textbf{46.0}\\
 \cline{2-9}
 & NI-TI-FGSM & 65.2 & 59.0 & 59.1 & ~~99.3* & 35.5 & 33.3 & 24.3\\
 & VNI-TI-FGSM & \textbf{76.3} & \textbf{73.3} & \textbf{73.5} & \textbf{~~99.6*} & \textbf{59.3} & \textbf{56.0} & \textbf{47.9}\\
\hline
\end{tabular}
\end{center}
\vspace{-0.5em}
\caption{The success rates (\%) on seven models in the single model setting by various gradient-based iterative attacks enhanced by Translation-Invariant Method.}
\label{tab:TIM}
\end{table*}
